NEPTUNE: Network- and GPU-aware Management of Serverless Functions at the Edge

Nowadays a wide range of applications is constrained by low-latency requirements that cloud infrastructures cannot meet. Multi-access Edge Computing (MEC) has been proposed as the reference architecture for executing applications closer to users and reduce latency, but new challenges arise: edge nodes are resource-constrained, the workload can vary significantly since users are nomadic, and task complexity is increasing (e.g., machine learning inference). To overcome these problems, the paper presents NEPTUNE, a serverless-based framework for managing complex MEC solutions. NEPTUNE i) places functions on edge nodes according to user locations, ii) avoids the saturation of single nodes, iii) exploits GPUs when available, and iv) allocates resources (CPU cores) dynamically to meet foreseen execution times. A prototype, built on top of K3S, was used to evaluate NEPTUNE on a set of experiments that demonstrate a significant reduction in terms of response time, network overhead, and resource consumption compared to three state-of-the-art approaches.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> acmart_bib_old.tex <==
@inproceedings{DBLP:conf/ispass/FelterFRR15,
  author    = {Wes Felter and
               Alexandre Ferreira and
               Ram Rajamony and
               Juan Rubio},
  title     = {An updated performance comparison of virtual machines and Linux containers},
  booktitle = {2015 {IEEE} International Symposium on Performance Analysis of Systems
               and Software, {ISPASS} 2015, Philadelphia, PA, USA, March 29-31, 2015},
  pages     = {171--172},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/ISPASS.2015.7095802},
  doi       = {10.1109/ISPASS.2015.7095802},
  timestamp = {Mon, 03 Aug 2020 15:48:48 +0200},
  biburl    = {https://dblp.org/rec/conf/ispass/FelterFRR15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/percom/TerefeLHFO16,
  author    = {Mati B. Terefe and
               Heezin Lee and
               Nojung Heo and
               Geoffrey Charles Fox and
               Sangyoon Oh},
  title     = {Energy-efficient multisite offloading policy using Markov decision
               process for mobile cloud computing},
  journal   = {Pervasive Mob. Comput.},
  volume    = {27},
  pages     = {75--89},
  year      = {2016},
  url       = {https://doi.org/10.1016/j.pmcj.2015.10.008},
  doi       = {10.1016/j.pmcj.2015.10.008},
  timestamp = {Sat, 22 Feb 2020 19:17:57 +0100},
  biburl    = {https://dblp.org/rec/journals/percom/TerefeLHFO16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/mlsys/MattsonCDCMPTWB20,
  author    = {Peter Mattson and
               Christine Cheng and
               Gregory F. Diamos and
               Cody Coleman and
               Paulius Micikevicius and
               David A. Patterson and
               Hanlin Tang and
               Gu{-}Yeon Wei and
               Peter Bailis and
               Victor Bittorf and
               David Brooks and
               Dehao Chen and
               Debo Dutta and
               Udit Gupta and
               Kim M. Hazelwood and
               Andy Hock and
               Xinyuan Huang and
               Daniel Kang and
               David Kanter and
               Naveen Kumar and
               Jeffery Liao and
               Deepak Narayanan and
               Tayo Oguntebi and
               Gennady Pekhimenko and
               Lillian Pentecost and
               Vijay Janapa Reddi and
               Taylor Robie and
               Tom St. John and
               Carole{-}Jean Wu and
               Lingjie Xu and
               Cliff Young and
               Matei Zaharia},
  editor    = {Inderjit S. Dhillon and
               Dimitris S. Papailiopoulos and
               Vivienne Sze},
  title     = {MLPerf Training Benchmark},
  booktitle = {Proceedings of Machine Learning and Systems 2020, MLSys 2020, Austin,
               TX, USA, March 2-4, 2020},
  publisher = {mlsys.org},
  year      = {2020},
  url       = {https://proceedings.mlsys.org/book/309.pdf},
  timestamp = {Thu, 18 Jun 2020 15:48:04 +0200},
  biburl    = {https://dblp.org/rec/conf/mlsys/MattsonCDCMPTWB20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/uemcom/VermaQF17,
  author    = {Abhishek Verma and
               Hussam Qassim and
               David Feinzimer},
  title     = {Residual squeeze {CNDS} deep learning {CNN} model for very large scale
               places image recognition},
  booktitle = {8th {IEEE} Annual Ubiquitous Computing, Electronics and Mobile Communication
               Conference, {UEMCON} 2017, New York City, NY, USA, October 19-21,
               2017},
  pages     = {463--469},
  publisher = {{IEEE}},
  year      = {2017},
  url       = {https://doi.org/10.1109/UEMCON.2017.8248975},
  doi       = {10.1109/UEMCON.2017.8248975},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/conf/uemcom/VermaQF17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/conext/ChoSMMR16,
  author    = {Junguk Cho and
               Karthikeyan Sundaresan and
               Rajesh Mahindra and
               Jacobus E. van der Merwe and
               Sampath Rangarajan},
  editor    = {Athina Markopoulou and
               Michalis Faloutsos and
               Vyas Sekar and
               Dejan Kostic},
  title     = {{ACACIA:} Context-aware Edge Computing for Continuous Interactive
               Applications over Mobile Networks},
  booktitle = {Proceedings of the 12th International on Conference on emerging Networking
               EXperiments and Technologies, CoNEXT 2016, Irvine, California, USA,
               December 12-15, 2016},
  pages     = {375--389},
  publisher = {{ACM}},
  year      = {2016},
  url       = {https://doi.org/10.1145/2999572.2999604},
  doi       = {10.1145/2999572.2999604},
  timestamp = {Tue, 06 Nov 2018 16:58:31 +0100},
  biburl    = {https://dblp.org/rec/conf/conext/ChoSMMR16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/wc/ZhangCZMXHYW19,
  author    = {Xu Zhang and
               Hao Chen and
               Yangchao Zhao and
               Zhan Ma and
               Yiling Xu and
               Haojun Huang and
               Hao Yin and
               Dapeng Oliver Wu},
  title     = {Improving Cloud Gaming Experience through Mobile Edge Computing},
  journal   = {{IEEE} Wirel. Commun.},
  volume    = {26},
  number    = {4},
  pages     = {178--183},
  year      = {2019},
  url       = {https://doi.org/10.1109/MWC.2019.1800440},
  doi       = {10.1109/MWC.2019.1800440},
  timestamp = {Tue, 24 Mar 2020 08:54:54 +0100},
  biburl    = {https://dblp.org/rec/journals/wc/ZhangCZMXHYW19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pieee/LiuLTYWS19,
  author    = {Shaoshan Liu and
               Liangkai Liu and
               Jie Tang and
               Bo Yu and
               Yifan Wang and
               Weisong Shi},
  title     = {Edge Computing for Autonomous Driving: Opportunities and Challenges},
  journal   = {Proc. {IEEE}},
  volume    = {107},
  number    = {8},
  pages     = {1697--1716},
  year      = {2019},
  url       = {https://doi.org/10.1109/JPROC.2019.2915983},
  doi       = {10.1109/JPROC.2019.2915983},
  timestamp = {Fri, 02 Oct 2020 14:42:45 +0200},
  biburl    = {https://dblp.org/rec/journals/pieee/LiuLTYWS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hpdc/WangAS21,
  author    = {Bin Wang and
               Ahmed Ali{-}Eldin and
               Prashant J. Shenoy},
  editor    = {Erwin Laure and
               Stefano Markidis and
               Ana Lucia Verbanescu and
               Jay F. Lofstead},
  title     = {LaSS: Running Latency Sensitive Serverless Computations at the Edge},
  booktitle = {{HPDC} '21: The 30th International Symposium on High-Performance Parallel
               and Distributed Computing, Virtual Event, Sweden, June 21-25, 2021},
  pages     = {239--251},
  publisher = {{ACM}},
  year      = {2021},
  url       = {https://doi.org/10.1145/3431379.3460646},
  doi       = {10.1145/3431379.3460646},
  timestamp = {Wed, 30 Jun 2021 16:55:43 +0200},
  biburl    = {https://dblp.org/rec/conf/hpdc/WangAS21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1902-03383,
  author     = {Eric Jonas and
                Johann Schleier{-}Smith and
                Vikram Sreekanti and
                Chia{-}che Tsai and
                Anurag Khandelwal and
                Qifan Pu and
                Vaishaal Shankar and
                Joao Carreira and
                Karl Krauth and
                Neeraja Jayant Yadwadkar and
                Joseph E. Gonzalez and
                Raluca Ada Popa and
                Ion Stoica and
                David A. Patterson},
  title      = {Cloud Programming Simplified: {A} Berkeley View on Serverless Computing},
  journal    = {CoRR},
  volume     = {abs/1902.03383},
  year       = {2019},
  url        = {http://arxiv.org/abs/1902.03383},
  eprinttype = {arXiv},
  eprint     = {1902.03383},
  timestamp  = {Tue, 21 May 2019 18:03:40 +0200},
  biburl     = {https://dblp.org/rec/journals/corr/abs-1902-03383.bib},
  bibsource  = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/globecom/Al-SaadehWSTL18,
  author    = {Osama Al{-}Saadeh and
               Gustav Wikstrom and
               Joachim Sachs and
               Ilaria Thibault and
               David Lister},
  title     = {End-to-End Latency and Reliability Performance of 5G in London},
  booktitle = {{IEEE} Global Communications Conference, {GLOBECOM} 2018, Abu Dhabi,
               United Arab Emirates, December 9-13, 2018},
  pages     = {1--6},
  publisher = {{IEEE}},
  year      = {2018},
  url       = {https://doi.org/10.1109/GLOCOM.2018.8647379},
  doi       = {10.1109/GLOCOM.2018.8647379},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/globecom/Al-SaadehWSTL18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/imc/LiYKZ10,
  author    = {Ang Li and
               Xiaowei Yang and
               Srikanth Kandula and
               Ming Zhang},
  editor    = {Mark Allman},
  title     = {CloudCmp: comparing public cloud providers},
  booktitle = {Proceedings of the 10th {ACM} {SIGCOMM} Internet Measurement Conference,
               {IMC} 2010, Melbourne, Australia - November 1-3, 2010},
  pages     = {1--14},
  publisher = {{ACM}},
  year      = {2010},
  url       = {https://doi.org/10.1145/1879141.1879143},
  doi       = {10.1145/1879141.1879143},
  timestamp = {Thu, 02 Jul 2020 17:46:32 +0200},
  biburl    = {https://dblp.org/rec/conf/imc/LiYKZ10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/middleware/SilvaFP20,
  author    = {Paulo Silva and
               Daniel Fireman and
               Thiago Emmanuel Pereira},
  editor    = {Dilma Da Silva and
               R{\"{u}}diger Kapitza},
  title     = {Prebaking Functions to Warm the Serverless Cold Start},
  booktitle = {Middleware '20: 21st International Middleware Conference, Delft, The
               Netherlands, December 7-11, 2020},
  pages     = {1--13},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3423211.3425682},
  doi       = {10.1145/3423211.3425682},
  timestamp = {Tue, 15 Dec 2020 14:30:24 +0100},
  biburl    = {https://dblp.org/rec/conf/middleware/SilvaFP20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iccS/CampmanySEMVL16,
  author    = {Victor Campmany and
               Sergio Silva and
               Antonio Espinosa and
               Juan Carlos Moure and
               David V{\'{a}}zquez and
               Antonio M. L{\'{o}}pez},
  editor    = {Michelle Connolly},
  title     = {GPU-based Pedestrian Detection for Autonomous Driving},
  booktitle = {International Conference on Computational Science 2016, {ICCS} 2016,
               6-8 June 2016, San Diego, California, {USA}},
  series    = {Procedia Computer Science},
  volume    = {80},
  pages     = {2377--2381},
  publisher = {Elsevier},
  year      = {2016},
  url       = {https://doi.org/10.1016/j.procs.2016.05.455},
  doi       = {10.1016/j.procs.2016.05.455},
  timestamp = {Thu, 08 Jul 2021 16:04:01 +0200},
  biburl    = {https://dblp.org/rec/conf/iccS/CampmanySEMVL16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hotedge/Biookaghazadeh018,
  author    = {Saman Biookaghazadeh and
               Ming Zhao and
               Fengbo Ren},
  editor    = {Irfan Ahmad and
               Swaminathan Sundararaman},
  title     = {Are FPGAs Suitable for Edge Computing?},
  booktitle = {{USENIX} Workshop on Hot Topics in Edge Computing, HotEdge 2018, Boston,
               MA, July 10, 2018},
  publisher = {{USENIX} Association},
  year      = {2018},
  url       = {https://www.usenix.org/conference/hotedge18/presentation/biookaghazadeh},
  timestamp = {Fri, 04 Jun 2021 11:57:43 +0200},
  biburl    = {https://dblp.org/rec/conf/hotedge/Biookaghazadeh018.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/access/GuptaJ15,
  author    = {Akhil Gupta and
               Rakesh Kumar Jha},
  title     = {A Survey of 5G Network: Architecture and Emerging Technologies},
  journal   = {{IEEE} Access},
  volume    = {3},
  pages     = {1206--1232},
  year      = {2015},
  url       = {https://doi.org/10.1109/ACCESS.2015.2461602},
  doi       = {10.1109/ACCESS.2015.2461602},
  timestamp = {Wed, 25 Sep 2019 17:49:03 +0200},
  biburl    = {https://dblp.org/rec/journals/access/GuptaJ15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{driverless_cars_need_for_data_is_sparking_a_new_space_race,
  author = {Keith Naughton},
  title  = {Driverless Cars Need for Data Is Sparking a New Space Race},
  year   = 2021,
  url    = {https://www.bloomberg.com/news/articles/2021-09-17/carmakers-look-to-satellites-for-future-of-self-driving-vehicles},
  note   = {Accessed: 2021-11-17}
}

@inproceedings{DBLP:conf/icdm/XieSL11,
  author    = {Jierui Xie and
               Boleslaw K. Szymanski and
               Xiaoming Liu},
  editor    = {Myra Spiliopoulou and
               Haixun Wang and
               Diane J. Cook and
               Jian Pei and
               Wei Wang and
               Osmar R. Za{\"{\i}}ane and
               Xindong Wu},
  title     = {{SLPA:} Uncovering Overlapping Communities in Social Networks via
               a Speaker-Listener Interaction Dynamic Process},
  booktitle = {Data Mining Workshops (ICDMW), 2011 {IEEE} 11th International Conference
               on, Vancouver, BC, Canada, December 11, 2011},
  pages     = {344--349},
  publisher = {{IEEE} Computer Society},
  year      = {2011},
  url       = {https://doi.org/10.1109/ICDMW.2011.154},
  doi       = {10.1109/ICDMW.2011.154},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icdm/XieSL11.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icsa/BaresiQ20,
  author    = {Luciano Baresi and
               Giovanni Quattrocchi},
  title     = {{COCOS:} {A} Scalable Architecture for Containerized Heterogeneous
               Systems},
  booktitle = {2020 {IEEE} International Conference on Software Architecture, {ICSA}
               2020, Salvador, Brazil, March 16-20, 2020},
  pages     = {103--113},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/ICSA47634.2020.00018},
  doi       = {10.1109/ICSA47634.2020.00018},
  timestamp = {Sat, 06 Jun 2020 14:44:43 +0200},
  biburl    = {https://dblp.org/rec/conf/icsa/BaresiQ20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/globecom/GrimaldiPPSS15,
  author    = {Domenico Grimaldi and
               Valerio Persico and
               Antonio Pescap{\`{e}} and
               Alessandro Salvi and
               Stefania Santini},
  title     = {A Feedback-Control Approach for Resource Management in Public Clouds},
  booktitle = {2015 {IEEE} Global Communications Conference, {GLOBECOM} 2015, San
               Diego, CA, USA, December 6-10, 2015},
  pages     = {1--7},
  publisher = {{IEEE}},
  year      = {2015},
  url       = {https://doi.org/10.1109/GLOCOM.2014.7417016},
  doi       = {10.1109/GLOCOM.2014.7417016},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/globecom/GrimaldiPPSS15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icsoc/BaresiMQ19,
  author    = {Luciano Baresi and
               Danilo Filgueira Mendon{\c{c}}a and
               Giovanni Quattrocchi},
  editor    = {Sami Yangui and
               Ismael Bouassida Rodriguez and
               Khalil Drira and
               Zahir Tari},
  title     = {{PAPS:} {A} Framework for Decentralized Self-management at the Edge},
  booktitle = {Service-Oriented Computing - 17th International Conference, {ICSOC}
               2019, Toulouse, France, October 28-31, 2019, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {11895},
  pages     = {508--522},
  publisher = {Springer},
  year      = {2019},
  url       = {https://doi.org/10.1007/978-3-030-33702-5\_39},
  doi       = {10.1007/978-3-030-33702-5\_39},
  timestamp = {Thu, 14 Oct 2021 10:19:48 +0200},
  biburl    = {https://dblp.org/rec/conf/icsoc/BaresiMQ19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/usenix/WangLZRS18,
  author    = {Liang Wang and
               Mengyuan Li and
               Yinqian Zhang and
               Thomas Ristenpart and
               Michael M. Swift},
  editor    = {Haryadi S. Gunawi and
               Benjamin Reed},
  title     = {Peeking Behind the Curtains of Serverless Platforms},
  booktitle = {2018 {USENIX} Annual Technical Conference, {USENIX} {ATC} 2018, Boston,
               MA, USA, July 11-13, 2018},
  pages     = {133--146},
  publisher = {{USENIX} Association},
  year      = {2018},
  url       = {https://www.usenix.org/conference/atc18/presentation/wang-liang},
  timestamp = {Mon, 01 Feb 2021 08:43:54 +0100},
  biburl    = {https://dblp.org/rec/conf/usenix/WangLZRS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/computer/KephartC03,
  author    = {Jeffrey O. Kephart and
               David M. Chess},
  title     = {The Vision of Autonomic Computing},
  journal   = {Computer},
  volume    = {36},
  number    = {1},
  pages     = {41--50},
  year      = {2003},
  url       = {https://doi.org/10.1109/MC.2003.1160055},
  doi       = {10.1109/MC.2003.1160055},
  timestamp = {Wed, 12 Aug 2020 10:29:29 +0200},
  biburl    = {https://dblp.org/rec/journals/computer/KephartC03.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/IEEEcloud/DutreilhRMMT10,
  author    = {Xavier Dutreilh and
               Nicolas Rivierre and
               Aur{\'{e}}lien Moreau and
               Jacques Malenfant and
               Isis Truck},
  title     = {From Data Center Resource Allocation to Control Theory and Back},
  booktitle = {{IEEE} International Conference on Cloud Computing, {CLOUD} 2010,
               Miami, FL, USA, 5-10 July, 2010},
  pages     = {410--417},
  publisher = {{IEEE} Computer Society},
  year      = {2010},
  url       = {https://doi.org/10.1109/CLOUD.2010.55},
  doi       = {10.1109/CLOUD.2010.55},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/conf/IEEEcloud/DutreilhRMMT10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/eurosys/RzadcaFSZBKNSWH20,
  author    = {Krzysztof Rzadca and
               Pawel Findeisen and
               Jacek Swiderski and
               Przemyslaw Zych and
               Przemyslaw Broniek and
               Jarek Kusmierek and
               Pawel Nowak and
               Beata Strack and
               Piotr Witusowski and
               Steven Hand and
               John Wilkes},
  editor    = {Angelos Bilas and
               Kostas Magoutis and
               Evangelos P. Markatos and
               Dejan Kostic and
               Margo I. Seltzer},
  title     = {Autopilot: workload autoscaling at Google},
  booktitle = {EuroSys '20: Fifteenth EuroSys Conference 2020, Heraklion, Greece,
               April 27-30, 2020},
  pages     = {16:1--16:16},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3342195.3387524},
  doi       = {10.1145/3342195.3387524},
  timestamp = {Thu, 10 Sep 2020 09:33:09 +0200},
  biburl    = {https://dblp.org/rec/conf/eurosys/RzadcaFSZBKNSWH20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/jnca/LiuLSCCC17,
  author    = {Chunhong Liu and
               Chuanchang Liu and
               Yanlei Shang and
               Shiping Chen and
               Bo Cheng and
               Junliang Chen},
  title     = {An adaptive prediction approach based on workload pattern discrimination
               in the cloud},
  journal   = {J. Netw. Comput. Appl.},
  volume    = {80},
  pages     = {35--44},
  year      = {2017},
  url       = {https://doi.org/10.1016/j.jnca.2016.12.017},
  doi       = {10.1016/j.jnca.2016.12.017},
  timestamp = {Mon, 24 Feb 2020 15:56:26 +0100},
  biburl    = {https://dblp.org/rec/journals/jnca/LiuLSCCC17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icsoc/BaresiQR21,
  author    = {Luciano Baresi and
               Giovanni Quattrocchi and
               Nicholas Rasi},
  editor    = {Hakim Hacid and
               Odej Kao and
               Massimo Mecella and
               Naouel Moha and
               Hye{-}young Paik},
  title     = {Resource Management for TensorFlow Inference},
  booktitle = {Service-Oriented Computing - 19th International Conference, {ICSOC}
               2021, Virtual Event, November 22-25, 2021, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {13121},
  pages     = {238--253},
  publisher = {Springer},
  year      = {2021},
  url       = {https://doi.org/10.1007/978-3-030-91431-8\_15},
  doi       = {10.1007/978-3-030-91431-8\_15},
  timestamp = {Fri, 19 Nov 2021 12:08:15 +0100},
  biburl    = {https://dblp.org/rec/conf/icsoc/BaresiQR21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tjs/KhalidAPII18,
  author    = {Yasir Noman Khalid and
               Muhammad Aleem and
               Radu Prodan and
               Muhammad Azhar Iqbal and
               Muhammad Arshad Islam},
  title     = {E-OSched: a load balancing scheduler for heterogeneous multicores},
  journal   = {J. Supercomput.},
  volume    = {74},
  number    = {10},
  pages     = {5399--5431},
  year      = {2018},
  url       = {https://doi.org/10.1007/s11227-018-2435-1},
  doi       = {10.1007/s11227-018-2435-1},
  timestamp = {Fri, 22 May 2020 13:27:37 +0200},
  biburl    = {https://dblp.org/rec/journals/tjs/KhalidAPII18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ccece/KelkarD21,
  author    = {Anupa Kelkar and
               Chris Dick},
  title     = {A {GPU} Hyperconverged Platform for 5G vRAN and Multi - Access Edge
               Computing},
  booktitle = {34th {IEEE} Canadian Conference on Electrical and Computer Engineering,
               {CCECE} 2021, Virtual Event, September 12-17, 2021},
  pages     = {1--6},
  publisher = {{IEEE}},
  year      = {2021},
  url       = {https://doi.org/10.1109/CCECE53047.2021.9569133},
  doi       = {10.1109/CCECE53047.2021.9569133},
  timestamp = {Thu, 04 Nov 2021 08:10:20 +0100},
  biburl    = {https://dblp.org/rec/conf/ccece/KelkarD21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/access/PhamFHPLLHD20,
  author    = {Quoc{-}Viet Pham and
               Fang Fang and
               Vu Nguyen Ha and
               Md. Jalil Piran and
               Mai Le and
               Long Bao Le and
               Won{-}Joo Hwang and
               Zhiguo Ding},
  title     = {A Survey of Multi-Access Edge Computing in 5G and Beyond: Fundamentals,
               Technology Integration, and State-of-the-Art},
  journal   = {{IEEE} Access},
  volume    = {8},
  pages     = {116974--117017},
  year      = {2020},
  url       = {https://doi.org/10.1109/ACCESS.2020.3001277},
  doi       = {10.1109/ACCESS.2020.3001277},
  timestamp = {Thu, 06 Aug 2020 21:46:42 +0200},
  biburl    = {https://dblp.org/rec/journals/access/PhamFHPLLHD20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/infocom/PoularakisLTTT19,
  author    = {Konstantinos Poularakis and
               Jaime Llorca and
               Antonia Maria Tulino and
               Ian J. Taylor and
               Leandros Tassiulas},
  title     = {Joint Service Placement and Request Routing in Multi-cell Mobile Edge
               Computing Networks},
  booktitle = {2019 {IEEE} Conference on Computer Communications, {INFOCOM} 2019,
               Paris, France, April 29 - May 2, 2019},
  pages     = {10--18},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/INFOCOM.2019.8737385},
  doi       = {10.1109/INFOCOM.2019.8737385},
  timestamp = {Sun, 25 Jul 2021 11:53:48 +0200},
  biburl    = {https://dblp.org/rec/conf/infocom/PoularakisLTTT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tsc/ZhuA12,
  author    = {Qian Zhu and
               Gagan Agrawal},
  title     = {Resource Provisioning with Budget Constraints for Adaptive Applications
               in Cloud Environments},
  journal   = {{IEEE} Trans. Serv. Comput.},
  volume    = {5},
  number    = {4},
  pages     = {497--511},
  year      = {2012},
  url       = {https://doi.org/10.1109/TSC.2011.61},
  doi       = {10.1109/TSC.2011.61},
  timestamp = {Tue, 01 Dec 2020 17:43:07 +0100},
  biburl    = {https://dblp.org/rec/journals/tsc/ZhuA12.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/grid/Lorido-BotranML14,
  author    = {Tania Lorido{-}Botran and
               Jos{\'{e}} Miguel{-}Alonso and
               Jos{\'{e}} Antonio Lozano},
  title     = {A Review of Auto-scaling Techniques for Elastic Applications in Cloud
               Environments},
  journal   = {J. Grid Comput.},
  volume    = {12},
  number    = {4},
  pages     = {559--592},
  year      = {2014},
  url       = {https://doi.org/10.1007/s10723-014-9314-7},
  doi       = {10.1007/s10723-014-9314-7},
  timestamp = {Tue, 06 Jun 2017 22:25:21 +0200},
  biburl    = {https://dblp.org/rec/journals/grid/Lorido-BotranML14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/csur/QuCB18,
  author    = {Chenhao Qu and
               Rodrigo N. Calheiros and
               Rajkumar Buyya},
  title     = {Auto-Scaling Web Applications in Clouds: {A} Taxonomy and Survey},
  journal   = {{ACM} Comput. Surv.},
  volume    = {51},
  number    = {4},
  pages     = {73:1--73:33},
  year      = {2018},
  url       = {https://doi.org/10.1145/3148149},
  doi       = {10.1145/3148149},
  timestamp = {Sat, 08 Jan 2022 02:23:16 +0100},
  biburl    = {https://dblp.org/rec/journals/csur/QuCB18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/IEEEcloud/YazdanovF14,
  author    = {Lenar Yazdanov and
               Christof Fetzer},
  title     = {Lightweight Automatic Resource Scaling for Multi-tier Web Applications},
  booktitle = {2014 {IEEE} 7th International Conference on Cloud Computing, Anchorage,
               AK, USA, June 27 - July 2, 2014},
  pages     = {466--473},
  publisher = {{IEEE} Computer Society},
  year      = {2014},
  url       = {https://doi.org/10.1109/CLOUD.2014.69},
  doi       = {10.1109/CLOUD.2014.69},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/conf/IEEEcloud/YazdanovF14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tcc/JiaCL17,
  author    = {Mike Jia and
               Jiannong Cao and
               Weifa Liang},
  title     = {Optimal Cloudlet Placement and User to Cloudlet Allocation in Wireless
               Metropolitan Area Networks},
  journal   = {{IEEE} Trans. Cloud Comput.},
  volume    = {5},
  number    = {4},
  pages     = {725--737},
  year      = {2017},
  url       = {https://doi.org/10.1109/TCC.2015.2449834},
  doi       = {10.1109/TCC.2015.2449834},
  timestamp = {Sun, 21 Jun 2020 17:41:48 +0200},
  biburl    = {https://dblp.org/rec/journals/tcc/JiaCL17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pe/UrgaonkarWHZCL15,
  author    = {Rahul Urgaonkar and
               Shiqiang Wang and
               Ting He and
               Murtaza Zafer and
               Kevin S. Chan and
               Kin K. Leung},
  title     = {Dynamic service migration and workload scheduling in edge-clouds},
  journal   = {Perform. Evaluation},
  volume    = {91},
  pages     = {205--228},
  year      = {2015},
  url       = {https://doi.org/10.1016/j.peva.2015.06.013},
  doi       = {10.1016/j.peva.2015.06.013},
  timestamp = {Thu, 11 Mar 2021 15:48:35 +0100},
  biburl    = {https://dblp.org/rec/journals/pe/UrgaonkarWHZCL15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/infocom/TongLG16,
  author    = {Liang Tong and
               Yong Li and
               Wei Gao},
  title     = {A hierarchical edge cloud architecture for mobile computing},
  booktitle = {35th Annual {IEEE} International Conference on Computer Communications,
               {INFOCOM} 2016, San Francisco, CA, USA, April 10-14, 2016},
  pages     = {1--9},
  publisher = {{IEEE}},
  year      = {2016},
  url       = {https://doi.org/10.1109/INFOCOM.2016.7524340},
  doi       = {10.1109/INFOCOM.2016.7524340},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/infocom/TongLG16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/sensors/Leyva-PupoSC19,
  author    = {Irian Leyva{-}Pupo and
               Alejandro Santoyo{-}Gonz{\'{a}}lez and
               Cristina Cervell{\'{o}}{-}Pastor},
  title     = {A Framework for the Joint Placement of Edge Service Infrastructure
               and User Plane Functions for 5G},
  journal   = {Sensors},
  volume    = {19},
  number    = {18},
  pages     = {3975},
  year      = {2019},
  url       = {https://doi.org/10.3390/s19183975},
  doi       = {10.3390/s19183975},
  timestamp = {Sat, 30 May 2020 19:58:14 +0200},
  biburl    = {https://dblp.org/rec/journals/sensors/Leyva-PupoSC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2108-13222,
  author    = {David Bermbach and
               Jonathan Bader and
               Jonathan Hasenburg and
               Tobias Pfandzelter and
               Lauritz Thamsen},
  title     = {AuctionWhisk: Using an Auction-Inspired Approach for Function Placement
               in Serverless Fog Platforms},
  journal   = {CoRR},
  volume    = {abs/2108.13222},
  year      = {2021},
  url       = {https://arxiv.org/abs/2108.13222},
  eprinttype = {arXiv},
  eprint    = {2108.13222},
  timestamp = {Thu, 02 Sep 2021 14:42:29 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2108-13222.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/infocom/TanHLL17,
  author    = {Haisheng Tan and
               Zhenhua Han and
               Xiang{-}Yang Li and
               Francis C. M. Lau},
  title     = {Online job dispatching and scheduling in edge-clouds},
  booktitle = {2017 {IEEE} Conference on Computer Communications, {INFOCOM} 2017,
               Atlanta, GA, USA, May 1-4, 2017},
  pages     = {1--9},
  publisher = {{IEEE}},
  year      = {2017},
  url       = {https://doi.org/10.1109/INFOCOM.2017.8057116},
  doi       = {10.1109/INFOCOM.2017.8057116},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/infocom/TanHLL17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/iotj/YangHHHCG21,
  author    = {Guisong Yang and
               Ling Hou and
               Xingyu He and
               Daojing He and
               Sammy Chan and
               Mohsen Guizani},
  title     = {Offloading Time Optimization via Markov Decision Process in Mobile-Edge
               Computing},
  journal   = {{IEEE} Internet Things J.},
  volume    = {8},
  number    = {4},
  pages     = {2483--2493},
  year      = {2021},
  url       = {https://doi.org/10.1109/JIOT.2020.3033285},
  doi       = {10.1109/JIOT.2020.3033285},
  timestamp = {Tue, 02 Mar 2021 11:25:16 +0100},
  biburl    = {https://dblp.org/rec/journals/iotj/YangHHHCG21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/sensors/MutichiroT021,
  author    = {Briytone Mutichiro and
               Minh{-}Ngoc Tran and
               Young{-}Han Kim},
  title     = {QoS-Based Service-Time Scheduling in the IoT-Edge Cloud},
  journal   = {Sensors},
  volume    = {21},
  number    = {17},
  pages     = {5797},
  year      = {2021},
  url       = {https://doi.org/10.3390/s21175797},
  doi       = {10.3390/s21175797},
  timestamp = {Thu, 16 Sep 2021 18:04:38 +0200},
  biburl    = {https://dblp.org/rec/journals/sensors/MutichiroT021.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/complexity/BabarKDAHK21,
  author    = {Mohammad Babar and
               Muhammad Sohail Khan and
               Ahmad Din and
               Farman Ali and
               Usman Habib and
               Kyung Sup Kwak},
  title     = {Intelligent Computation Offloading for IoT Applications in Scalable
               Edge Computing Using Artificial Bee Colony Optimization},
  journal   = {Complex.},
  volume    = {2021},
  pages     = {5563531:1--5563531:12},
  year      = {2021},
  url       = {https://doi.org/10.1155/2021/5563531},
  doi       = {10.1155/2021/5563531},
  timestamp = {Tue, 01 Jun 2021 08:35:43 +0200},
  biburl    = {https://dblp.org/rec/journals/complexity/BabarKDAHK21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tvt/Al-HabobDAM20,
  author    = {Ahmed A. Al{-}Habob and
               Octavia A. Dobre and
               Ana Garc{\'{\i}}a Armada and
               Sami Muhaidat},
  title     = {Task Scheduling for Mobile Edge Computing Using Genetic Algorithm
               and Conflict Graphs},
  journal   = {{IEEE} Trans. Veh. Technol.},
  volume    = {69},
  number    = {8},
  pages     = {8805--8819},
  year      = {2020},
  url       = {https://doi.org/10.1109/TVT.2020.2995146},
  doi       = {10.1109/TVT.2020.2995146},
  timestamp = {Wed, 26 Aug 2020 11:03:56 +0200},
  biburl    = {https://dblp.org/rec/journals/tvt/Al-HabobDAM20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icc/SunA16,
  author    = {Xiang Sun and
               Nirwan Ansari},
  title     = {{PRIMAL:} PRofIt Maximization Avatar pLacement for mobile edge computing},
  booktitle = {2016 {IEEE} International Conference on Communications, {ICC} 2016,
               Kuala Lumpur, Malaysia, May 22-27, 2016},
  pages     = {1--6},
  publisher = {{IEEE}},
  year      = {2016},
  url       = {https://doi.org/10.1109/ICC.2016.7511131},
  doi       = {10.1109/ICC.2016.7511131},
  timestamp = {Fri, 09 Apr 2021 18:40:55 +0200},
  biburl    = {https://dblp.org/rec/conf/icc/SunA16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/access/Oleghe21,
  author    = {Omogbai Oleghe},
  title     = {Container Placement and Migration in Edge Computing: Concept and Scheduling
               Models},
  journal   = {{IEEE} Access},
  volume    = {9},
  pages     = {68028--68043},
  year      = {2021},
  url       = {https://doi.org/10.1109/ACCESS.2021.3077550},
  doi       = {10.1109/ACCESS.2021.3077550},
  timestamp = {Tue, 01 Jun 2021 08:34:47 +0200},
  biburl    = {https://dblp.org/rec/journals/access/Oleghe21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/nca/ZhouWWQ20,
  author    = {Ao Zhou and
               Shangguang Wang and
               Shaohua Wan and
               Lianyong Qi},
  title     = {{LMM:} latency-aware micro-service mashup in mobile edge computing
               environment},
  journal   = {Neural Comput. Appl.},
  volume    = {32},
  number    = {19},
  pages     = {15411--15425},
  year      = {2020},
  url       = {https://doi.org/10.1007/s00521-019-04693-w},
  doi       = {10.1007/s00521-019-04693-w},
  timestamp = {Tue, 20 Oct 2020 18:27:29 +0200},
  biburl    = {https://dblp.org/rec/journals/nca/ZhouWWQ20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/wowmom/TasiopoulosAPP18,
  author    = {Argyrios G. Tasiopoulos and
               Onur Ascigil and
               Ioannis Psaras and
               George Pavlou},
  title     = {Edge-MAP: Auction Markets for Edge Resource Provisioning},
  booktitle = {19th {IEEE} International Symposium on "A World of Wireless, Mobile
               and Multimedia Networks", WoWMoM 2018, Chania, Greece, June 12-15,
               2018},
  pages     = {14--22},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {https://doi.org/10.1109/WoWMoM.2018.8449792},
  doi       = {10.1109/WoWMoM.2018.8449792},
  timestamp = {Wed, 16 Oct 2019 14:14:55 +0200},
  biburl    = {https://dblp.org/rec/conf/wowmom/TasiopoulosAPP18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icsoc/BaresiHQT21,
  author    = {Luciano Baresi and
               Davide Yi Xian Hu and
               Giovanni Quattrocchi and
               Luca Terracciano},
  editor    = {Hakim Hacid and
               Odej Kao and
               Massimo Mecella and
               Naouel Moha and
               Hye{-}young Paik},
  title     = {{KOSMOS:} Vertical and Horizontal Resource Autoscaling for Kubernetes},
  booktitle = {Service-Oriented Computing - 19th International Conference, {ICSOC}
               2021, Virtual Event, November 22-25, 2021, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {13121},
  pages     = {821--829},
  publisher = {Springer},
  year      = {2021},
  url       = {https://doi.org/10.1007/978-3-030-91431-8\_59},
  doi       = {10.1007/978-3-030-91431-8\_59},
  timestamp = {Fri, 19 Nov 2021 12:08:15 +0100},
  biburl    = {https://dblp.org/rec/conf/icsoc/BaresiHQT21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icccs/JahaniLCAA019,
  author    = {Arezoo Jahani and
               Marco Lattuada and
               Michele Ciavotta and
               Danilo Ardagna and
               Edoardo Amaldi and
               Li Zhang},
  title     = {Optimizing on-demand GPUs in the Cloud for Deep Learning Applications
               Training},
  booktitle = {2019 4th International Conference on Computing, Communications and
               Security (ICCCS), Rome, Italy, October 10-12, 2019},
  pages     = {1--8},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/CCCS.2019.8888151},
  doi       = {10.1109/CCCS.2019.8888151},
  timestamp = {Fri, 27 Dec 2019 21:29:33 +0100},
  biburl    = {https://dblp.org/rec/conf/icccs/JahaniLCAA019.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hpdc/YehCC20,
  author    = {Ting{-}An Yeh and
               Hung{-}Hsin Chen and
               Jerry Chou},
  editor    = {Manish Parashar and
               Vladimir Vlassov and
               David E. Irwin and
               Kathryn Mohror},
  title     = {KubeShare: {A} Framework to Manage GPUs as First-Class and Shared
               Resources in Container Cloud},
  booktitle = {{HPDC} '20: The 29th International Symposium on High-Performance Parallel
               and Distributed Computing, Stockholm, Sweden, June 23-26, 2020},
  pages     = {173--184},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3369583.3392679},
  doi       = {10.1145/3369583.3392679},
  timestamp = {Fri, 11 Jun 2021 08:37:45 +0200},
  biburl    = {https://dblp.org/rec/conf/hpdc/YehCC20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/asplos/LinZHSHTM18,
  author    = {Shih{-}Chieh Lin and
               Yunqi Zhang and
               Chang{-}Hong Hsu and
               Matt Skach and
               Md. Enamul Haque and
               Lingjia Tang and
               Jason Mars},
  editor    = {Xipeng Shen and
               James Tuck and
               Ricardo Bianchini and
               Vivek Sarkar},
  title     = {The Architectural Implications of Autonomous Driving: Constraints
               and Acceleration},
  booktitle = {Proceedings of the Twenty-Third International Conference on Architectural
               Support for Programming Languages and Operating Systems, {ASPLOS}
               2018, Williamsburg, VA, USA, March 24-28, 2018},
  pages     = {751--766},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3173162.3173191},
  doi       = {10.1145/3173162.3173191},
  timestamp = {Wed, 23 Jun 2021 15:34:31 +0200},
  biburl    = {https://dblp.org/rec/conf/asplos/LinZHSHTM18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ictc/KimLLNTC20,
  author    = {Namkyu Kim and
               Yunseong Lee and
               Chunghyun Lee and
               The{-}Vi Nguyen and
               Van{-}Dat Tuong and
               Sungrae Cho},
  title     = {GPU-specific Task Offloading in the Mobile Edge Computing Network},
  booktitle = {International Conference on Information and Communication Technology
               Convergence, {ICTC} 2020, Jeju Island, Korea (South), October 21-23,
               2020},
  pages     = {1874--1876},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/ICTC49870.2020.9289354},
  doi       = {10.1109/ICTC49870.2020.9289354},
  timestamp = {Tue, 02 Feb 2021 11:06:24 +0100},
  biburl    = {https://dblp.org/rec/conf/ictc/KimLLNTC20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/fgcs/BellendorfM20,
  author    = {Julian Bellendorf and
               Zolt{\'{a}}n {\'{A}}d{\'{a}}m Mann},
  title     = {Classification of optimization problems in fog computing},
  journal   = {Future Gener. Comput. Syst.},
  volume    = {107},
  pages     = {158--176},
  year      = {2020},
  url       = {https://doi.org/10.1016/j.future.2020.01.036},
  doi       = {10.1016/j.future.2020.01.036},
  timestamp = {Tue, 21 Apr 2020 08:56:39 +0200},
  biburl    = {https://dblp.org/rec/journals/fgcs/BellendorfM20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hpdc/FuerstASS20,
  author    = {Alexander Fuerst and
               Ahmed Ali{-}Eldin and
               Prashant J. Shenoy and
               Prateek Sharma},
  editor    = {Manish Parashar and
               Vladimir Vlassov and
               David E. Irwin and
               Kathryn Mohror},
  title     = {Cloud-scale VM-deflation for Running Interactive Applications On Transient
               Servers},
  booktitle = {{HPDC} '20: The 29th International Symposium on High-Performance Parallel
               and Distributed Computing, Stockholm, Sweden, June 23-26, 2020},
  pages     = {53--64},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3369583.3392675},
  doi       = {10.1145/3369583.3392675},
  timestamp = {Tue, 11 Aug 2020 17:19:32 +0200},
  biburl    = {https://dblp.org/rec/conf/hpdc/FuerstASS20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/services/PaladeKC19,
  author    = {Andrei Palade and
               Aqeel Kazmi and
               Siobh{\'{a}}n Clarke},
  editor    = {Carl K. Chang and
               Peter Chen and
               Michael Goul and
               Katsunori Oyama and
               Stephan Reiff{-}Marganiec and
               Yanchun Sun and
               Shangguang Wang and
               Zhongjie Wang},
  title     = {An Evaluation of Open Source Serverless Computing Frameworks Support
               at the Edge},
  booktitle = {2019 {IEEE} World Congress on Services, {SERVICES} 2019, Milan, Italy,
               July 8-13, 2019},
  pages     = {206--211},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/SERVICES.2019.00057},
  doi       = {10.1109/SERVICES.2019.00057},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/conf/services/PaladeKC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/IEEEcloud/RattihalliGLT19,
  author    = {Gourav Rattihalli and
               Madhusudhan Govindaraju and
               Hui Lu and
               Devesh Tiwari},
  editor    = {Elisa Bertino and
               Carl K. Chang and
               Peter Chen and
               Ernesto Damiani and
               Michael Goul and
               Katsunori Oyama},
  title     = {Exploring Potential for Non-Disruptive Vertical Auto Scaling and Resource
               Estimation in Kubernetes},
  booktitle = {12th {IEEE} International Conference on Cloud Computing, {CLOUD} 2019,
               Milan, Italy, July 8-13, 2019},
  pages     = {33--40},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/CLOUD.2019.00018},
  doi       = {10.1109/CLOUD.2019.00018},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/conf/IEEEcloud/RattihalliGLT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/access/JiangCGZW19,
  author    = {Congfeng Jiang and
               Xiaolan Cheng and
               Honghao Gao and
               Xin Zhou and
               Jian Wan},
  title     = {Toward Computation Offloading in Edge Computing: {A} Survey},
  journal   = {{IEEE} Access},
  volume    = {7},
  pages     = {131543--131558},
  year      = {2019},
  url       = {https://doi.org/10.1109/ACCESS.2019.2938660},
  doi       = {10.1109/ACCESS.2019.2938660},
  timestamp = {Thu, 07 Nov 2019 09:19:02 +0100},
  biburl    = {https://dblp.org/rec/journals/access/JiangCGZW19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/IEEEcloud/SubediHKR21,
  author    = {Piyush Subedi and
               Jianwei Hao and
               In Kee Kim and
               Lakshmish Ramaswamy},
  editor    = {Claudio Agostino Ardagna and
               Carl K. Chang and
               Ernesto Daminai and
               Rajiv Ranjan and
               Zhongjie Wang and
               Robert Ward and
               Jia Zhang and
               Wensheng Zhang},
  title     = {{AI} Multi-Tenancy on Edge: Concurrent Deep Learning Model Executions
               and Dynamic Model Placements on Edge Devices},
  booktitle = {14th {IEEE} International Conference on Cloud Computing, {CLOUD} 2021,
               Chicago, IL, USA, September 5-10, 2021},
  pages     = {31--42},
  publisher = {{IEEE}},
  year      = {2021},
  url       = {https://doi.org/10.1109/CLOUD53861.2021.00016},
  doi       = {10.1109/CLOUD53861.2021.00016},
  timestamp = {Mon, 15 Nov 2021 17:41:59 +0100},
  biburl    = {https://dblp.org/rec/conf/IEEEcloud/SubediHKR21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/infocom/GuoXYY16,
  author    = {Songtao Guo and
               Bin Xiao and
               Yuanyuan Yang and
               Yang Yang},
  title     = {Energy-efficient dynamic offloading and resource scheduling in mobile
               cloud computing},
  booktitle = {35th Annual {IEEE} International Conference on Computer Communications,
               {INFOCOM} 2016, San Francisco, CA, USA, April 10-14, 2016},
  pages     = {1--9},
  publisher = {{IEEE}},
  year      = {2016},
  url       = {https://doi.org/10.1109/INFOCOM.2016.7524497},
  doi       = {10.1109/INFOCOM.2016.7524497},
  timestamp = {Tue, 31 Mar 2020 16:35:50 +0200},
  biburl    = {https://dblp.org/rec/conf/infocom/GuoXYY16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/cacm/CastroIMS19,
  author    = {Paul C. Castro and
               Vatche Ishakian and
               Vinod Muthusamy and
               Aleksander Slominski},
  title     = {The rise of serverless computing},
  journal   = {Commun. {ACM}},
  volume    = {62},
  number    = {12},
  pages     = {44--54},
  year      = {2019},
  url       = {https://doi.org/10.1145/3368454},
  doi       = {10.1145/3368454},
  timestamp = {Thu, 05 Dec 2019 10:17:53 +0100},
  biburl    = {https://dblp.org/rec/journals/cacm/CastroIMS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1903-12221,
  author    = {Ping{-}Min Lin and
               Alex Glikson},
  title     = {Mitigating Cold Starts in Serverless Platforms: {A} Pool-Based Approach},
  journal   = {CoRR},
  volume    = {abs/1903.12221},
  year      = {2019},
  url       = {http://arxiv.org/abs/1903.12221},
  eprinttype = {arXiv},
  eprint    = {1903.12221},
  timestamp = {Tue, 02 Apr 2019 12:29:45 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1903-12221.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{9326369,
  author  = {Ascigil, Onur and Tasiopoulos, Argyrios and Phan, Truong Khoa and Sourlas, Vasilis and Psaras, Ioannis and Pavlou, George},
  journal = {IEEE Transactions on Services Computing},
  title   = {Resource Provisioning and Allocation in Function-as-a-Service Edge-Clouds (Early Access)},
  year    = {2021},
  volume  = {},
  number  = {},
  doi     = {10.1109/TSC.2021.3052139}
}

@misc{kubernetes_vpa,
  key    = {Kubernetes VPA},
  title  = {Vertical Pod Autoscaler},
  year   = 2021,
  url    = {https://github.com/kubernetes/autoscaler/tree/master/vertical-pod-autoscaler},
  note   = {Accessed: 2022-01-13}
}

@inproceedings{DBLP:conf/kivs/KalmbachBKPJH19,
  author    = {Patrick Kalmbach and
               Andreas Blenk and
               Wolfgang Kellerer and
               Rastin Pries and
               Michael Jarschel and
               Marco Hoffmann},
  title     = {{GPU} Accelerated Planning and Placement of Edge Clouds},
  booktitle = {2019 International Conference on Networked Systems, NetSys 2019, Munich,
               Germany, March 18-21, 2019},
  pages     = {1--3},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/NetSys.2019.8854495},
  doi       = {10.1109/NetSys.2019.8854495},
  timestamp = {Wed, 16 Oct 2019 14:14:53 +0200},
  biburl    = {https://dblp.org/rec/conf/kivs/KalmbachBKPJH19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@incollection{DBLP:books/daglib/p/WohlinHH06,
  author    = {Claes Wohlin and
               Martin H{\"{o}}st and
               Kennet Henningsson},
  editor    = {Emilia Mendes and
               Nile Mosley},
  title     = {Empirical Research Methods in Web and Software Engineering},
  booktitle = {Web Engineering},
  pages     = {409--430},
  publisher = {Springer},
  year      = {2006},
  url       = {https://doi.org/10.1007/3-540-28218-1\_13},
  doi       = {10.1007/3-540-28218-1\_13},
  timestamp = {Wed, 14 Jun 2017 20:28:58 +0200},
  biburl    = {https://dblp.org/rec/books/daglib/p/WohlinHH06.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/recsys/FelicioniDCBHBD20,
  author    = {Nicol{\`{o}} Felicioni and
               Andrea Donati and
               Luca Conterio and
               Luca Bartoccioni and
               Davide Yi Xian Hu and
               Cesare Bernardis and
               Maurizio Ferrari Dacrema},
  title     = {Multi-Objective Blended Ensemble For Highly Imbalanced Sequence Aware
               Tweet Engagement Prediction},
  booktitle = {RecSys Challenge '20: Proceedings of the Recommender Systems Challenge
               2020, Virtual Event Brazil, September, 2020},
  pages     = {29--33},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3415959.3415998},
  doi       = {10.1145/3415959.3415998},
  timestamp = {Mon, 03 Jan 2022 22:40:00 +0100},
  biburl    = {https://dblp.org/rec/conf/recsys/FelicioniDCBHBD20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1911-01296,
  author    = {Hossein Shafiei and
               Ahmad Khonsari},
  title     = {Serverless Computing: Opportunities and Challenges},
  journal   = {CoRR},
  volume    = {abs/1911.01296},
  year      = {2019},
  url       = {http://arxiv.org/abs/1911.01296},
  eprinttype = {arXiv},
  eprint    = {1911.01296},
  timestamp = {Mon, 11 Nov 2019 18:38:09 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1911-01296.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/closer/QuintK18,
  author    = {Peter{-}Christian Quint and
               Nane Kratzke},
  editor    = {V{\'{\i}}ctor M{\'{e}}ndez Mu{\~{n}}oz and
               Donald Ferguson and
               Markus Helfert and
               Claus Pahl},
  title     = {Towards a Lightweight Multi-Cloud {DSL} for Elastic and Transferable
               Cloud-native Applications},
  booktitle = {Proceedings of the 8th International Conference on Cloud Computing
               and Services Science, {CLOSER} 2018, Funchal, Madeira, Portugal, March
               19-21, 2018},
  pages     = {400--408},
  publisher = {SciTePress},
  year      = {2018},
  url       = {https://doi.org/10.5220/0006683804000408},
  doi       = {10.5220/0006683804000408},
  timestamp = {Fri, 27 Mar 2020 08:54:54 +0100},
  biburl    = {https://dblp.org/rec/conf/closer/QuintK18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ccbd/ShiWXC16,
  author    = {Shaohuai Shi and
               Qiang Wang and
               Pengfei Xu and
               Xiaowen Chu},
  title     = {Benchmarking State-of-the-Art Deep Learning Software Tools},
  booktitle = {7th International Conference on Cloud Computing and Big Data, {CCBD}
               2016, Macau, China, November 16-18, 2016},
  pages     = {99--104},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CCBD.2016.029},
  doi       = {10.1109/CCBD.2016.029},
  timestamp = {Thu, 28 Oct 2021 13:52:50 +0200},
  biburl    = {https://dblp.org/rec/conf/ccbd/ShiWXC16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{DBLP:journals/rfc/rfc3626,
  author    = {Thomas Heide Clausen and
               Philippe Jacquet},
  title     = {Optimized Link State Routing Protocol {(OLSR)}},
  journal   = {{RFC}},
  volume    = {3626},
  pages     = {1--75},
  year      = {2003},
  url       = {https://doi.org/10.17487/RFC3626},
  doi       = {10.17487/RFC3626},
  timestamp = {Tue, 14 May 2019 10:03:45 +0200},
  biburl    = {https://dblp.org/rec/journals/rfc/rfc3626.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/rfc/rfc777,
  author    = {Jon Postel},
  title     = {Internet Control Message Protocol},
  journal   = {{RFC}},
  volume    = {777},
  pages     = {1--14},
  year      = {1981},
  url       = {https://doi.org/10.17487/RFC0777},
  doi       = {10.17487/RFC0777},
  timestamp = {Tue, 14 May 2019 10:03:28 +0200},
  biburl    = {https://dblp.org/rec/journals/rfc/rfc777.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/fgcs/KumarS18,
  author    = {Jitendra Kumar and
               Ashutosh Kumar Singh},
  title     = {Workload prediction in cloud using artificial neural network and adaptive
               differential evolution},
  journal   = {Future Gener. Comput. Syst.},
  volume    = {81},
  pages     = {41--52},
  year      = {2018},
  url       = {https://doi.org/10.1016/j.future.2017.10.047},
  doi       = {10.1016/j.future.2017.10.047},
  timestamp = {Fri, 13 Nov 2020 09:24:30 +0100},
  biburl    = {https://dblp.org/rec/journals/fgcs/KumarS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/IEEEcloud/LinKW18,
  author    = {Wei{-}Tsung Lin and
               Chandra Krintz and
               Rich Wolski},
  title     = {Tracing Function Dependencies across Clouds},
  booktitle = {11th {IEEE} International Conference on Cloud Computing, {CLOUD} 2018,
               San Francisco, CA, USA, July 2-7, 2018},
  pages     = {253--260},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {https://doi.org/10.1109/CLOUD.2018.00039},
  doi       = {10.1109/CLOUD.2018.00039},
  timestamp = {Wed, 16 Oct 2019 14:14:54 +0200},
  biburl    = {https://dblp.org/rec/conf/IEEEcloud/LinKW18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/SnoekLA12,
  author    = {Jasper Snoek and
               Hugo Larochelle and
               Ryan P. Adams},
  editor    = {Peter L. Bartlett and
               Fernando C. N. Pereira and
               Christopher J. C. Burges and
               L{\'{e}}on Bottou and
               Kilian Q. Weinberger},
  title     = {Practical Bayesian Optimization of Machine Learning Algorithms},
  booktitle = {Advances in Neural Information Processing Systems 25: 26th Annual
               Conference on Neural Information Processing Systems 2012. Proceedings
               of a meeting held December 3-6, 2012, Lake Tahoe, Nevada, United States},
  pages     = {2960--2968},
  year      = {2012},
  url       = {https://proceedings.neurips.cc/paper/2012/hash/05311655a15b75fab86956663e1819cd-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:23 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/SnoekLA12.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/europar/BaresiQ18,
  author    = {Luciano Baresi and
               Giovanni Quattrocchi},
  editor    = {Gabriele Mencagli and
               Dora B. Heras and
               Valeria Cardellini and
               Emiliano Casalicchio and
               Emmanuel Jeannot and
               Felix Wolf and
               Antonio Salis and
               Claudio Schifanella and
               Ravi Reddy Manumachu and
               Laura Ricci and
               Marco Beccuti and
               Laura Antonelli and
               Jos{\'{e}} Daniel Garc{\'{\i}}a S{\'{a}}nchez and
               Stephen L. Scott},
  title     = {Towards Vertically Scalable Spark Applications},
  booktitle = {Euro-Par 2018: Parallel Processing Workshops - Euro-Par 2018 International
               Workshops, Turin, Italy, August 27-28, 2018, Revised Selected Papers},
  series    = {Lecture Notes in Computer Science},
  volume    = {11339},
  pages     = {106--118},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-10549-5\_9},
  doi       = {10.1007/978-3-030-10549-5\_9},
  timestamp = {Fri, 27 Dec 2019 21:26:53 +0100},
  biburl    = {https://dblp.org/rec/conf/europar/BaresiQ18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

==> sections/implementation.tex <==
\section{Prototype}\label{sec:implementation}

This section presents the prototype\footnote{Available at \url{https://github.com/deib-polimi/edge-autoscaler}.} of \approach built on top of Kubernetes, the de-facto standard container orchestrator, and compatible with OpenFaaS function specifications, a well-known open-source serverless platform.
The prototype only uses the native Kubernetes APIs, and it was developed on top of K3s\footnote{https://k3s.io}, a lightweight distribution of Kubernetes optimized for edge computing with a smaller memory footprint. K3s is fully compatible with Kubernetes APIs, tools, and programming model.

\subsection{Kubernetes}

Kubernetes adopts a distributed architecture with a master node (or \textit{K3s-server} in K3s) that manages a set of workers (or \textit{K3s-agents} in K3s) in charge of running containers. The master node can be replicated to increase availability; workers use a daemon called \textit{kubelet} to communicate with the master node(s).

Kubernetes uses \textit{resources} to represent both the underlying infrastructure and applications. Some resources are built-in, but additional ones can be defined by users as Custom Resource Definitions (CRDs).
Resource \textit{pod} is the smallest unit that can be deployed in the cluster and it wraps one or more containers into a single isolated environment. Users can manually configure the minimum and maximum amount of resources that can be used by a pod. For pods replicated across multiple instances, Kubernetes provides means to distribute the workload to replicas using different strategies such as round-robin or strategies based on predefined weights.

Kubernetes allows the creation of automated control loops using the so-called \textit{controller pattern}\footnote{\url{https://kubernetes.io/docs/concepts/architecture/controller/##controller-pattern}}. Users declare goals (e.g., the desired response time) using Kubernetes resources, \textit{controllers} are then in charge of accomplishing the objectives by operating on the deployment (e.g., by scaling the number of pod replicas). %Built-in controllers use built-in resources, while custom controllers employ CRDs. In their decision process, 
Controllers can also exploit the Kubernetes monitoring system (i.e., the \textit{metric server}) or custom ones (e.g., Prometheus\footnote{https://github.com/kubernetes-sigs/prometheus-adapter}).

Users or controllers can trigger the deployment of new pods. To do so, Kubernetes employs a scheduler that is in charge of identifying a node that could host the new pod. While the built-in scheduler, namely \textit{kube-scheduler}, adopts a scoring algorithm to decide (e.g., based on CPU consumption, memory), custom schedulers can also be defined by users.

Finally, to cope with hardware heterogeneity, Kubernetes offers a framework called \textit{device plugin} to enable the support of new devices such as GPUs. The built-in plugin assigns a GPU to a single pod at a time, which holds the ownership for its whole lifetime.

\subsection{Architecture}

Figure \ref{fig:implementation:architecture} shows the architecture of our prototype. The prototype assumes that each node corresponds to a Kubernetes worker (or a K3s-agent) running in the cluster. Each control level is embedded in a dedicated component that implements the controller pattern. In particular, component \textit{Topology controller} dynamically splits the network using the SLPA algorithm, component \textit{Community controller} is in charge of generating the function placement and the routing policies for each community, and component \textit{Node controller} embeds all the PI controllers that perform dynamic resource allocation at \nodelevel.

Since available monitoring solutions do not provide means to monitor and collect the fine-grained metrics required by \approach, we implemented a custom monitoring system that exploits the \textit{Sidecar pattern}\footnote{https://docs.microsoft.com/en-us/azure/architecture/patterns/sidecar}. This pattern aims to create two or more containers in the same pod where one embeds the application logic, and the others perform non-functional tasks such as monitoring, logging, and configuration without requiring modifications to the running application.
Thus, the prototype employs a custom lightweight proxy (as sidecar) that is automatically injected inside all function pods and intercepts required metrics. Monitoring proxies push the collected data into component \textit{Metrics Database}, which is used by the controllers to be aware of the performance of the system.


\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{images/architecture.pdf}
    \caption{\approach architecture. \luc{Perch\`e non c'\`e nessuna relazione tra FUNCTION 1 GPU e AWS DEVICE PLUGIN e NVIDIA MPS?}}
    \label{fig:implementation:architecture}
    \Description{Prototype architecture.}
\end{figure}


The Topology controller periodically checks for changes in the node network (e.g., when a node is added or removed) and executes the SLPA algorithm to reorganize nodes in communities. \luc{Diciamo da qualche parte ogni quanto avviene? \`E periodo o basato su eventi?}\lt{Per Davide e Giovanni: lo ho inserito alla fine di sezione 2, ci conviene inserirlo qui?}

\luc{Stacco}
New functions can be deployed by using a \luc{dedicated} textit{Function} resource (i.e., a CRD) provided by OpenFaaS. 
Once the \textit{Function} resource is created, the Community controller addresses the new function in the placement process.
Since communities are independent, one instance of the function will be created in each community. As said, the placement takes into account the functions that require GPUs and creates pods able to exploit the dedicated hardware.
Whenever a new placement is computed, \approach routing policies are written in an additional CRD named \textit{Community Schedule}, which will then be read by the load balancers.


State-of-the-art load balancers are not designed to handle frequent changes in routing policies and they must be restarted every time the internal configuration is modified.
For this reason, we developed a custom load balancer that is able to periodically change its routing policies without service interruption. the prototype deploys an instance of this load balancer on each node.

When the traffic for a deployed function $f$ reaches a node $j$, the load balancer (running on $j$) collects the arrival rate $\lambda_{f,j}$ and the average response time $rt_{f,j}$, and stores these data into the Metrics Database. With these data, the Community controller may i) move the instances closer to the traffic source, ii) adjust function instances according to the workload, and iii) properly update routing policies by using the formulation described in Section~\ref{sec:second-level}.

The heuristic used by kube-scheduler to deploy containers could interfere with the logic of Community controllers. For this reason, our prototype uses a custom scheduler, implemented as a sub-component of Community controller, which directly enacts the newly computed placements.

The prototype supports a seamless evolution of the system.
Old instances are not deleted until the new ones are ready to serve requests. Furthermore, the deletion occurs using graceful termination periods, giving time to all instances to finish serving pending requests.
Then, load balancers update their routing policies to guarantee service availability: whenever new routing policies are rolled out, the prototype waits until the new pods are available before replacing the old ones.

Each Node controller is in charge of scaling the cores associated with each function instance (vertical scaling).
The current standard distribution of Kubernetes does not allow one to change allocated resources without restarting pods, a process that sometimes can take minutes. This could compromise the \nodelevel, which would become incapable of handling bursty workloads.
As a result, the prototype augments Kubernetes with the \textit{Kubernetes Enhancement Proposal}  1287  that implements \textit{In-Place Pod Vertical Scaling}\footnote{https://github.com/kubernetes/enhancements/tree/master/keps/sig-node/1287-in-place-update-pod-resources} and allows pods' resources to be changed without restarts. This enables Node controllers to operate at faster pace.

To provide an effective usage of GPUs, the prototype uses \textit{nvidia-docker}, a container runtime that enables the usage of GPUs inside containers. \luc{E la relazione con device plugin descritto prima?}
However, by default, GPU access can be reserved to only one function instance at a time. This prevents the full exploitation of the GPU and limits the possible placements produced by Community controllers.
To solve this problem the prototype employs a device plugin\footnote{https://github.com/awslabs/aws-virtual-gpu-device-plugin} developed by Amazon that enables the fractional allocation of GPUs. In particular, the plugin makes use of the \textit{Nvidia Multi Process Service}\footnote{https://docs.nvidia.com/deploy/mps/index.html} (MPS), a runtime architecture designed to transparently allow GPUs to be shared among multiple processes (e.g., containers).

When available GPUs are not enough to carry out all requested computations, we create an additional container for the same function, but that only exploits CPUs  (as Function $1$ in  Figure~\ref{fig:implementation:architecture}). This replication is mandatory since the runtimes dedicated to GPU processing (e.g., TensorFlow serving\footnote{https://www.tensorflow.org/tfx/guide/serving}) do not allow the same container to exploit both GPUs and CPUs.

